Ultra Inertial Poser: Scalable Motion Capture and Tracking from Sparse Inertial Sensors and Ultra-Wideband Ranging

While camera-based capture systems remain the gold standard for recording human motion, learning-based tracking systems based on sparse wearable sensors are gaining popularity. Most commonly, they use inertial sensors, whose propensity for drift and jitter have so far limited tracking accuracy. In this paper, we propose Ultra Inertial Poser, a novel 3D full body pose estimation method that constrains drift and jitter in inertial tracking via inter-sensor distances. We estimate these distances across sparse sensor setups using a lightweight embedded tracker that augments inexpensive off-the-shelf 6D inertial measurement units with ultra-wideband radio-based ranging$-$dynamically and without the need for stationary reference anchors. Our method then fuses these inter-sensor distances with the 3D states estimated from each sensor Our graph-based machine learning model processes the 3D states and distances to estimate a person's 3D full body pose and translation. To train our model, we synthesize inertial measurements and distance estimates from the motion capture database AMASS. For evaluation, we contribute a novel motion dataset of 10 participants who performed 25 motion types, captured by 6 wearable IMU+UWB trackers and an optical motion capture system, totaling 200 minutes of synchronized sensor data (UIP-DB). Our extensive experiments show state-of-the-art performance for our method over PIP and TIP, reducing position error from $13.62$ to $10.65cm$ ($22\%$ better) and lowering jitter from $1.56$ to $0.055km/s^3$ (a reduction of $97\%$).

==> sec/0_abstract_shorter.tex <==
\begin{teaserfigure}
  \vspace{-2mm}
  \includegraphics[width=\textwidth]{figs/teaser_v1_christian-3.pdf}%
  \vspace{-2mm}
  \caption{Our method \emph{Ultra Inertial Poser} estimates 3D full body poses and global translation (i.e., SMPL parameters) from the inertial measurements on a sparse set of wearable sensors, augmented and stabilized by the estimated inter-sensor distances based on UWB ranging.
  Our lightweight standalone sensors stream \emph{raw IMU signals}, from which we estimate each tracker's 3D state and fuse it with acceleration and inter-sensor distances in a graph-based machine learning model for pose estimation.}
  \Description{This is the teaser figure for the article in four sections.
  The left-most image is a photograph of an individual walking outdoors wearing six wearable trackers placed on the head, back, wrists, and knees. The image next to it is a stylized outline of the person, with reference coordinates for each sensor $S_0$ to $S_5$ and lines connecting them illustrating inter-sensor distances. Next, is a detailed look of the sensor hardware, comprising an IMU, UWB module, and a case with a strap, alongside Velcro for attaching Optitrack markers. An AirTag is included for size reference. Finally, the right-most image shows the SMPL model estimated using data from the wearable sensors, depicting full-body pose and translation.
}
  \label{fig:teaser}
\end{teaserfigure}


\begin{abstract}

While camera-based capture systems remain the gold standard for recording human motion, learning-based tracking systems based on sparse wearable sensors are gaining popularity.
Most commonly, they use inertial sensors, whose propensity for drift and jitter have so far limited tracking accuracy.
In this paper, we propose \emph{Ultra Inertial Poser}, a novel 3D full body pose estimation method that constrains drift and jitter in inertial tracking via inter-sensor distances.
We estimate these distances across sparse sensor setups using a lightweight embedded tracker that augments inexpensive off-the-shelf 6D inertial measurement units with ultra-wideband radio-based ranging---dynamically and without the need for stationary reference anchors.
Our method then fuses these inter-sensor distances with the 3D states estimated from each sensor.
Our graph-based machine learning model processes the 3D states and distances to estimate a person's 3D full body pose and translation.
To train our model, we synthesize inertial measurements and distance estimates from the motion capture database AMASS.
For evaluation, we contribute a novel motion dataset of 10 participants who performed 25 motion types, captured by 6 wearable IMU+UWB trackers and an optical motion capture system, totaling 200 minutes of synchronized sensor data (UIP-DB).
%\ch{One sentence on final results.}
Our extensive experiments show state-of-the-art performance for our method over PIP and TIP, reducing position error from 13.62 to 10.65\,cm (22\% better) and lowering jitter from 1.56 to 0.055\,km/s$^3$ (a reduction of 97\%).

\begin{center}
~\\
\vspace{1mm}
UIP code, UIP-DB dataset, and hardware design:

\href{https://github.com/eth-siplab/UltraInertialPoser}{\texttt{\color{magenta}{https://github.com/eth-siplab/UltraInertialPoser}}}
\vspace{3mm}
\end{center}

\end{abstract}

